MP-Former: Mask-Piloted Transformer for Image Segmentation

We present a mask-piloted Transformer which improves masked-attention in Mask2Former for image segmentation. The improvement is based on our observation that Mask2Former suffers from inconsistent mask predictions between consecutive decoder layers, which leads to inconsistent optimization goals and low utilization of decoder queries. To address this problem, we propose a mask-piloted training approach, which additionally feeds noised ground-truth masks in masked-attention and trains the model to reconstruct the original ones. Compared with the predicted masks used in mask-attention, the ground-truth masks serve as a pilot and effectively alleviate the negative impact of inaccurate mask predictions in Mask2Former. Based on this technique, our \M achieves a remarkable performance improvement on all three image segmentation tasks (instance, panoptic, and semantic), yielding $+2.3$AP and $+1.6$mIoU on the Cityscapes instance and semantic segmentation tasks with a ResNet-50 backbone. Our method also significantly speeds up the training, outperforming Mask2Former with half of the number of training epochs on ADE20K with both a ResNet-50 and a Swin-L backbones. Moreover, our method only introduces little computation during training and no extra computation during inference. Our code will be released at \url{https://github.com/IDEA-Research/MP-Former}.

==> 00_abstract.tex <==
\begin{abstract}
% Abstract goes here.
\end{abstract}

==> 01_intro.tex <==
\section{Introduction}
\label{sec:intro}


==> 02_related.tex <==
\section{Related Work}
\label{sec:related}



==> 03_method.tex <==
\section{Method}
\label{sec:method}



==> 10_conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}



==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}


==> resources/images/analyze_match.tex <==
\begin{figure*}[h]
\centering
\subfigure[The predicted mask of the $0$th layer of Mask2Former.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_ori_0.png}
%\caption{fig1}
\end{minipage}%
}%
\subfigure[The predicted mask of the last layer of Mask2Former.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_ori_9.png}
%\caption{fig2}
\end{minipage}%
}%
\subfigure[The predicted mask of the $0$th layer of Mask DINO.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_m2f_0.png}
%\caption{fig2}
\end{minipage}
}%
\subfigure[The predicted mask of the last layer of Mask2 DINO.]{
\begin{minipage}[h]{0.25\linewidth}
\centering
\includegraphics[width=1in]{resources/images/match_m2f_9.png}
%\caption{fig2}
\end{minipage}
}%
\centering
\caption{(a)(b) are the $0$th and the last layer prediction of Mask2Former. Obviously the $2$ predictions of the same query are matched with different instances. (a) matches the rear vehicle and (b) matches the front vehicle.  (b)(c) shows those of our Mask DINO. The two predictions both match the front vehicle.}
\label{fig:analyze_match}
\end{figure*}


==> resources/images/framework.tex <==
\begin{figure}[h]
% \vspace{-0.8cm}
    \includegraphics[width=\columnwidth]{resources/images/compare_arch.pdf}
    % \graphics{resources/images/framework.pdf}
    % \fbox{resources/images/framework.pdf}
    \centering
    % \vspace{-0.5cm}
    \caption{ A comparison of Transformer decoder of our \M and Mask2Former. \M feeds extra queries and attention masks which are marked by dashed lines. The queries are taken as the class embedding of the GT categories and the attention masks are GT masks. Since we adopt multi-layer mask guide, we feed GT masks as attention masks not only in the first layer but also in subsequent layers. However, we did not feed class embeddings in multiple layers.}
    \label{fig:compare m2f}
    % \vspace{-0.8cm}
\end{figure}

==> resources/images/noise_analysis.tex <==
\begin{figure*}[ht]
\centering
\subfigure[]{
\begin{minipage}[h]{0.45\linewidth}
\centering
\includegraphics[height=3.0in]{resources/images/noise_analysis/shift.png}
\end{minipage}%
}%
\hspace{0.5in}
\subfigure[]{
\begin{minipage}[h]{0.4\linewidth}
\centering
\includegraphics[height=3.0in]{resources/images/noise_analysis/scaling.png}

\end{minipage}%
}%



\centering
\caption{(a)(b) Demonstration of shifting noise and scaling noise respectively. The blue and green crescent-shaped regions are examples of the original GT mask and noised GT mask respectively. The blue and green boxes are bounding box of the original GT mask and noised GT mask. $\lambda$ denotes the scales of the noises which are proportional to the size of the GT bounding boxes.}
\label{fig:noise_type_ana}
\end{figure*}

==> resources/images/theory_2.tex <==
\begin{figure}[h]
\vspace{-0.3cm}
    % \includegraphics[width=0.4\columnwidth]{resources/images/demo.pdf}
    % % \graphics{resources/images/framework.pdf}
    % % \fbox{resources/images/framework.pdf}
    % \centering
    % % \vspace{-0.5cm}
    % \caption{A demo}
    % \label{fig:demo}
%     \centering
% \subfigure[]{
% \begin{minipage}[h]{0.2\linewidth}
% \centering
% \includegraphics[width=2in]{resources/images/demo.pdf}
% %\caption{fig1}
% \end{minipage}%
% }%
% \hspace{0.7in}
\centering
% \subfigure[]{
\begin{minipage}[h]{1.0\linewidth}
\centering
\includegraphics[width=2.5in]{resources/images/demo.pdf}
%\caption{fig1}
\end{minipage}%
\caption{A demonstration of how our method works.}
\label{fig:demo}
% }%
    % \includegraphics[width=0.4\columnwidth]{resources/images/arch.pdf}
    % % \graphics{resources/images/framework.pdf}
    % % \fbox{resources/images/framework.pdf}
    % \centering
    % % \vspace{-0.5cm}
    % \caption{A demo}
    % \label{fig:arch}
    % \vspace{-0.8cm}
\end{figure}

==> resources/tables/boxhelpmask.tex <==
% \begin{table}[h]
% % \vspace{-.4cm}
%     \centering
%     %     \footnotesize
%     %         \renewcommand{\arraystretch}{1.6}
%     % \resizebox{\columnwidth}{!}{%
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     % \begin{tabular}{l|c|cccccc}
%     \begin{tabular}{l|c|c|ccccccc|c|c|c}
%     \midrule
%         \multicolumn{2}{c}{Tasks} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mask AP} &  \\
%          \scriptsize Box& \scriptsize Mask & & \\
%         \midrule
%         % Mask-RCNN & $400$ & Dense anchors  & $42.5$ & $48.2$ & $-$ & $-$ & $23.8$ & $45.0$ & $60.0$ & $207$ & $40$M & $21^{*}$ \\
%         % HTC \cite{chen2019hybrid}& $24$ & Dense anchors & $38.4$ & $42.3$ & $-$ & $-$ & $-$ & $-$ & $-$ &$441$ & $80$M & $5^{*}$ \\
%         % QueryInst &&&&&&&&&& \\
       
%         % \hline
       
        
%         % DINO-4scale    &36 & 900 queries & - &{50.5}& $-$ & $-$ & $-$ & $-$ & $-$&$279$ & $47$M & 24\\
%         % DINO-4scale    &36 & 300 queries & - &{49.6}& $-$ & $-$ & $-$ & $-$ & $-$ &$279$ & $47$M & 24\\
%         % \hline
%         % Mask2Former$^*$    &50 & 100 queries& {43.7} & 46.2$^{\dag}$ & $-$ & $-$ & $23.4$ & $47.2$ & $64.8$ &$226$ & $44$M & 9.7 \\
%         % Mask DINO    &50 & 100 queries  &{45.4} &{49.8} & $-$ & $-$ & $-$ & $-$ & $-$ &$-$ & $44$M & - \\
%         % Mask DINO    &50 & 300 queries  &\textbf{46.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.3)} &\textbf{50.5} & $68.9$ & $50.3$ & \textbf{26.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.6)} & $49.3$ & $65.5$ &$234$ & $44$M & - \\
%         %  \hline
%         % Mask2Former    &12 & 100 queries& {38.7} & -& $-$ & $-$ & $23.4$ & $47.2$ & $64.8$ &$226$ & $44$M & 9.7 \\
%         % Mask DINO    &12 & 300 queries  &\textbf{41.4}\fontsize{7.0pt}{\baselineskip}\selectfont{(+2.7)} &{44.5} & $-$ & $-$ & $-$ & $-$ & $-$ &$234$ & $44$M & - \\
%         \midrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     % \vspace{0.2cm}
%     \caption{Results for Mask DINO and other object detection and instance segmentation models with the ResNet-50 backbone on COCO \texttt{val2017}. We follow the common practice in DETR-like models to use 300 queries. $^*$ The performance of Mask2Former will degenerate when using 300 queries. $\dag$ indicates the box AP is generated from mask prediction.
%     % $^*$ indicates it is the test-dev result.
%     % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
%     % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
%     }
    
%     \label{tab:boxhelpmask}
%     % \vspace{-.4cm}
% \end{table}

==> resources/tables/helpandmatch.tex <==
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{minipage}[t]{0.5\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{cc|ccc}
    \toprule
    \multicolumn{2}{c}{Tasks} & \multicolumn{2}{c}{box AP} & \multirow{2}{*}{mask AP} \\
          Box&  Mask &12ep&50ep & \\
        \midrule
    \checkmark     &      &$\textbf{45.1}$& $50.1$ &- \\
     & \checkmark  & - && $43.3$   \\
    \checkmark     & \checkmark &$44.5$& $\textbf{50.5}$ & $\textbf{46.0}$     \\
    \bottomrule
\end{tabular}
\caption{Task comparison on COCO Val under 50-epoch setting with Resnet-50 backbone. We use the same model but train different tasks to verify the effectiveness of hybrid training.}
\label{tab:taskhelp}
\end{minipage}\hspace{8mm}
\begin{minipage}[t]{0.58\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|ccc}
    \toprule
    test layer & Mask DION & Mask2Former  \\
        \midrule
        layer 0 & $\textbf{39.6}$ & $1.1$     \\
        \midrule
        layer 3&$\textbf{44.0}$&$42.3$\\
     layer 6     &$\textbf{45.9}$    & $43.3$  \\
     layer 9  &  $\textbf{46.0}$    & ${43.7}$  \\
    
    \bottomrule
\end{tabular}
\caption{Effectiveness of our query selection for mask initialization. We evaluate the instance segmentation performance of different decoder layers of the same model on COCO val after training 50 epochs. "layer 0" means we do not use decoder and the results is directly got from encoder query selection.}
\label{tab:dec_test}
\end{minipage}
% \begin{minipage}[t]{0.5\textwidth}
% \makeatletter\def\@captype{table}
% \begin{tabular}{cccc}
%     \toprule
%     \multicolumn{2}{c}{Matching} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mask AP} \\
%           Box&  Mask & & \\
%         \midrule
%     \checkmark     &      & $44.4$ & $40.5$ \\
%      & \checkmark  & $40.2$ &$38.4$     \\
%     \checkmark & \checkmark     & $\textbf{44.5}$ & $\textbf{41.4}$      \\
%     \bottomrule
% \end{tabular}
% \caption{Matching method comparison on COCO Val under 12-epoch setting.}
% \label{sample-table}
% \end{minipage}
\end{adjustbox}

% \begin{minipage}[t]{0.48\textwidth}
% \makeatletter\def\@captype{table}
% \begin{tabular}{ccc}
%     \toprule
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
% \end{tabular}
% \caption{Sample table title}
% \label{sample-table}
% \end{minipage}
% \end{minipage}


==> resources/tables/main_ablation.tex <==
\begin{adjustbox}{width=1.0\textwidth,center}
    \begin{minipage}[t]{0.64\columnwidth}
\makeatletter\def\@captype{table}
\centering
    \begin{tabular}{c|ccc}
        \midrule
          & box AP & mask AP   \\
        \midrule
         Mask DINO (ours) & 44.5&\textbf{41.4} \\
         \midrule
         $-$ DINO Mask branch$^*$  & 49.5$^{\dag}$&35.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-5.7)}   \\
         $-$ Unified query selection for masks  & 43.6&40.3 \fontsize{7.0pt}{\baselineskip}\selectfont{(-1.1)}   \\
         $-$ Hybrid matching & 44.4 & 40.5 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.9)}   \\
        $-$ Mask denoising & 44.6&40.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.7)}    \\
        \midrule
    \end{tabular}
    \caption{Ablation comparison of the proposed components under \\12-epoch setting on COCO val. $^*$ indicates we use original DETR~\cite{carion2020end} segmentation branch with $300$ queries, where we follow DETR to finetune segmentation after finishing training detection. $^{\dag}$ the performance of detection drops ($49.6$ AP as shown in Table \ref{tab:instance} when only training detection) after training segmentation.
    }
    \label{tab:ablation}
    \end{minipage}\hspace{6mm}
%     \begin{minipage}[t]{0.5\textwidth}
% \makeatletter\def\@captype{table}
% \begin{tabular}{cccc}
%     \toprule
%     \multicolumn{2}{c}{Matching} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mask AP} \\
%           Box&  Mask & & \\
%         \midrule
%     \checkmark     &      & $44.4$ & $40.5$ \\
%      & \checkmark  & $40.2$ &$38.4$     \\
%     \checkmark & \checkmark     & $\textbf{44.5}$ & $\textbf{41.4}$      \\
%     \bottomrule
% \end{tabular}
% \caption{Matching method comparison on COCO Val under 12-epoch setting.}
% \label{sample-table}
% \end{minipage}
    \begin{minipage}[t]{0.39\columnwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{cc|cc}
    \toprule
    \multicolumn{2}{c}{Matching} & \multirow{2}{*}{box AP} & \multirow{2}{*}{mask AP} \\
          Box&  Mask & & \\
        \midrule
    \checkmark     &      & $44.4$ & $40.5$ \\
     & \checkmark  & $40.2$ &$38.4$     \\
    \checkmark & \checkmark     & $\textbf{44.5}$ & $\textbf{41.4}$      \\
    \bottomrule
\end{tabular}
\caption{Matching method comparison on COCO val under 12-epoch setting. We train both tasks together but use different matching method to verify the effectiveness of hybrid matching.}
\label{sample-table}
\end{minipage}
    \end{adjustbox}
    % \vspace{-.8cm}
% \end{table}
% \begin{table}[h]
% % \vspace{-0.4cm}
%     \centering
%     % \resizebox{\textwidth}{!}{%
%     \begin{adjustbox}{width=1.0\textwidth,center}
%     \begin{tabular}{l|cc|ccccccc}
%         \midrule
%         \#Row  & box AP & mask AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ \\
%         \midrule
%         1. Basic Mask DINO & Running \\
%         2. Row1 + Hybrid matching & Running   \\
%         % 1. Optimized DN-DETR &  No & & \checkmark  & $45.2$ & $61.6$ & $48.7$ & $27.2$ & $48.0$ & $59.6$\\
%         3. Row2 + Mask denoising & TODO 095    \\
%         % 3.  & Pure  &  & \checkmark  & $46.7$ & $63.9$ & $50.9$ & $29.8$ & $49.8$ & $61.3$\\
%         % 4. + Mask denoising & Mixed  &  &  & $47.0$ & $64.2$ & $51.0$ & $31.1$ & $50.1$ & $61.5$\\
%         % 4.  & Mixed  &  & \checkmark & $47.0$ & $65.1$ & $50.9$ & $28.9$ & $50.1$ & $62.0$\\
%         % 5. Row4+look forward twice  & Mixed  &  & \checkmark  & $47.4$ & $64.8$ & $51.6$ & $29.9$ & $50.8$ & $61.9$\\
%         4. {Mask DINO} (ours, Row3 + Unified query selection for masks)  & 44.5&41.4   \\
%         \midrule
%     \end{tabular}
%     \end{adjustbox}
%     \centering
%     \vspace{0.3cm}
%     \caption{Ablation comparison of the proposed algorithm components.
%     }
%     % \vspace{-0.1cm}
%     \label{tab:ablation}
%     \vspace{-.8cm}
% \end{table}

% \begin{minipage}[t]{0.4\textwidth}
% \makeatletter\def\@captype{table}
%     \begin{tabular}{cccccccccc}
%         \midrule
%           & box AP & mask AP & AP$_{50}$ & AP$_{75}$ & AP$_{S}$ & AP$_{M}$ & AP$_{L}$ \\
%         \midrule
%          Mask DINO & 44.5&\textbf{41.4} \\
%          \midrule
%          $-$ DINO Mask branch$^*$  & 49.5$^{\dag}$&35.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-5.7)}   \\
%          $-$ Unified query selection for masks  & 43.6&40.3 \fontsize{7.0pt}{\baselineskip}\selectfont{(-1.1)}   \\
%          $-$ Hybrid matching & 44.4 & 40.5 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.9)}   \\
%         $-$ Mask denoising & 44.6&40.7 \fontsize{7.0pt}{\baselineskip}\selectfont{(-0.7)}    \\
%         \midrule
%     \end{tabular}
%     % \caption{Ablation comparison of the proposed components under 12-epoch setting on COCO val. $^*$ indicates we use original DETR~\cite{carion2020end} segmentation branch with $300$ queries, where we follow DETR to finetune segmentation after finishing training detection. $^{\dag}$ the performance of detection drops ($49.6$ AP as shown in Table \ref{tab:instance} when only training detection) after training segmentation.
%     % }
%     \label{tab:ablation}
%     \end{minipage}


==> resources/tables/match_util_compare.tex <==
\begin{table}[]
\begin{tabular}{lllllllllll}
\midrule
 Layer Number                            &   & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8&9 \\\midrule
\multirow{2}{*}{Mask2Former} & Utility(\%)  & 38.1 & 65.5 & 70.8 & 73.5 & 78.5 & 81.1 & 83.2 & 83.2 &100  \\
                             & mean IoU(\%) & 23.0 & 50.3 & 59.5 & 69.7 & 70.1 & 69.9 & 78.6 & 76.3 & 76.0 \\\midrule
\multirow{2}{*}{ours}        & Utility(\%)  & 82.6 & 89.1 & 89.9 & 90.4 & 87.9 & 89.9 & 89.8 & 87.1&100 \\
                             & mean IoU(\%)  & 47.6  & 76.1 & 78.8 & 92.4 & 91.4 & 88.9 & 95.8 & 95.9 & 95.2\\\midrule
\end{tabular}
% \begin{tabular}{llllllllllll}
% \hline
% layer number           & 0    & 1    & 2    & 3    & 4    & 5    & 6    & 7    & 8    \\ \hline
% Query utility & 25.1 & 38.1 & 65.5 & 70.8 & 73.5 & 78.5 & 81.1 & 83.2 & 83.2  \\
% mean Iou & 23.0 & 50.3 & 59.5 & 69.7 & 70.1 & 69.9 & 78.6 & 76.3 & 76.0  \\\hline
% \M  & 35.2 & 82.6 & 89.1 & 89.9 & 90.4 & 87.9 & 89.9 & 89.8 & 87.1 & 100 \\ \hline
% \M  & 47.6  & 76.1 & 78.8 & 92.4 & 91.4 & 88.9 & 95.8 & 95.9 & 95.2 \\ \hline
% \end{tabular}
\caption{A comparison of the Layer wise utility and mean IoU of Mask2Former and our \M. The utility is the ratio of queries matched with GT masks that are matched with the same GT mask in the last layer. The IoU for a query is taken as the IoU of the predicted masks in $i$th and $(i+1)$th decoder layers. The mean IoU take average over all queries.}
\label{tab:util comp}
\end{table}

==> resources/tables/scaleandlayernum.tex <==
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{minipage}[t]{0.58\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|ccc}
    \toprule
   Feature scale & box AP & {mask AP} & FLOPs \\
        \midrule
    single scale(1/8)     &  Running    & Running  \\
     3 scales  & $50.5$ & $45.8$   \\
    4 scales & $50.5$ & $\textbf{46.0}$     \\
    \bottomrule
\end{tabular}
\caption{Multi-scale feature comparison on COCO Val under 50-epoch setting with Resnet-50 backbone.}
\label{sample-table}
\end{minipage}\hspace{10mm}
\begin{minipage}[t]{0.58\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|ccc}
    \toprule
   Decoder layer\# & box AP & {mask AP} & FLOPs \\
        \midrule
        3&$43.1$&$40.7$\\
     6     &$44.3$    & $41.1$  \\
     9  &  $44.5$    & $\textbf{41.4}$  \\
    12 & $44.8$ & $41.1$     \\
    \bottomrule
\end{tabular}
\caption{Decoder layer number comparison on COCO Val under 12-epoch setting.}
\label{tab:dec_layer}
\end{minipage}
\end{adjustbox}

% \begin{minipage}[t]{0.48\textwidth}
% \makeatletter\def\@captype{table}
% \begin{tabular}{ccc}
%     \toprule
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
% \end{tabular}
% \caption{Sample table title}
% \label{sample-table}
% \end{minipage}
% \end{minipage}


==> resources/tables/semantic.tex <==
\begin{adjustbox}{width=1.0\textwidth,center}
\begin{minipage}[t]{0.6\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|c|cc|c}
    \midrule
        Model&Backbone  & Iterations& Crop size &mIoU (s.s.)  \\
        \midrule
        Mask2Former&R50 &160k& $512$ & $47.2$   \\
          Mask3Former&R50   & 80k&$512$  &\textbf{47.4}\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.2)}\\
          Mask3Former&R50 &160k& $512$ & \textbf{48.1}\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.9)}\\
          \midrule
          Mask2Former&Swin-L &160k& $512$ & $56.2$   \\
          Mask3Former&Swin-L   & 80k&$512$  &\textbf{56.9}\fontsize{7.0pt}{\baselineskip}\selectfont{(+0.7)}
    \end{tabular}
    \centering
    % \vspace{0.2cm}
    \caption{Results for Mask3Former and other semantic segmentation models with the ResNet-50 backbone on ADE20K \texttt{val}.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    \label{tab:sematic}
\end{minipage}\hspace{18mm}
\begin{minipage}[t]{0.6\textwidth}
\makeatletter\def\@captype{table}
\centering
\begin{tabular}{c|c|c|c}
    \midrule
        Model  &Backbone& Iterations &mIoU (s.s.)  \\
        \midrule
        Mask2Former&R50 &90k & $79.4$   \\
          Mask3Former&R50   & 90k  &\textbf{81.0}\fontsize{7.0pt}{\baselineskip}\selectfont{(+1.6)}  \\
          \midrule
          Mask2Former&Swin-L &90k & $-$   \\
          Mask3Former&Swin-L   & 90k &\textbf{-}\fontsize{7.0pt}{\baselineskip}\selectfont{(-)}  
          
    \end{tabular}
    \centering
    % \vspace{0.2cm}
    \caption{Results for Mask3Former and other semantic segmentation models with the ResNet-50 backbone on Cityscapes \texttt{val}.
    % $^*$ indicates it is the test-dev result.
    % All DETR-like models except DETR use $300$ queries, while DETR uses $100$.
    % The models with superscript $^{*}$ use $3$ pattern embeddings as in Anchor DETR~\cite{wang2021anchor}.
    }
    
    
    \label{tab:sematic}
\end{minipage}
\end{adjustbox}

==> resources/tables/sota.tex <==
\begin{table}
% \vspace{-0.4cm}
    \centering
    \small
        \setlength\tabcolsep{2pt}
        \footnotesize
            \renewcommand{\arraystretch}{1.3}
    % \resizebox{}{!}{%
    % \resizebox{0.5\columnwidth}{!}{%
    % \resizebox{\columnwidth}{!}
    \begin{adjustbox}{width=1.0\textwidth,center}
    \begin{tabular}{c|c|c|c|c|c|cc|cc}
    % \begin{tabular}{c|c|c|c|c|c|c|ccc}
        
        \midrule
        \multirow{2}{*}{Method} & \multirow{2}{*}{Params} & \multirow{2}{*}{Backbone} & \multirow{2}{*}{\makecell{Backbone Pre-training \\ Dataset }} &  \multirow{2}{*}{\makecell{Detection Pre-training \\ Dataset }} &  \multirow{2}{*}{End-to-end}  & \multicolumn{2}{c|}{{ val}} & \multicolumn{2}{c}{{test}} \\
        & & & & && \scriptsize w/o TTA& \scriptsize w/ TTA &\scriptsize w/o TTA&\scriptsize w/ TTA \\
        \midrule
        \multicolumn{6}{c}{{\textbf{Instance segmentation on COCO}}}&\multicolumn{4}{c}{AP} \\
        \midrule
        % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
        Mask2Former & $216$M & SwinL & IN-22K-14M & -  &   & $50.1$ & $-$ & $50.4$ & $-$ \\
        Soft Teacher+SwinL~\cite{xu2021end} & $284$M & SwinL & IN-22K-14M & O365  &   &$51.9$ & $52.5$ & $-$ & $53.0$ \\
        SwinV2-G~\cite{liu2021swinv2} & $3.0$B & SwinV2-G & IN-22K-ext-70M~\cite{liu2021swinv2} & O365 &   & $53.4$ & $53.7$ & $-$ & $54.5$\\
        \hline
        MASK DINO(Ours) & $\textbf{218}$\textbf{M} & SwinL & IN-22K-14M & O365 &   & $\textbf{54.5}$ & $\textbf{-}$ & $\textbf{-}$ & $\textbf{-}$ \\
        \midrule
        \multicolumn{6}{c}{{\textbf{Panoptic segmentation on COCO}}}&\multicolumn{4}{c}{PQ} \\
        \midrule
        % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
        Mask2Former & $216$M & SwinL & IN-22K-14M & -  &   & $57.8$ & $-$ & $58.3$ & $-$ \\
        Panoptic SegFormer~ & $-$M & SwinL & IN-22K-14M & -  &   &$55.8$ & $-$ & $56.2$ & $-$ \\
        % SwinV2-G~\cite{liu2021swinv2} & $3.0$B & IN-22K-ext-70M~\cite{liu2021swinv2} & O365 &   & $61.9$ & $62.5$ & $-$ & $63.1$\\
        \hline
        MASK DINO(Ours) & $\textbf{218}$\textbf{M} & SwinL & IN-22K-14M & O365 &   & $\textbf{58.9}$ & $\textbf{-}$ & $\textbf{-}$ & $\textbf{-}$ \\
        \midrule
        \multicolumn{6}{c}{{\textbf{Semantic segmentation on ADE20K}}}&\multicolumn{4}{c}{mIoU} \\
        \midrule
        % SwinL~\cite{liu2021swin} & $284$M & IN-22K-14M & O365   & & $57.1$ & $58.0$ & $57.7$ & $58.7$ \\
        Mask2Former & $-$M & SwinL-FaPN & IN-22K-14M  & -  &   & $56.4$ & $57.7$ & $56.4$ & $57.7$ \\
        SeMask-L MSFaPN-Mask2Former~ & $-$M & SwinL-FaPN & IN-22K-14M & -  &   &$-$ & $58.2$ & $-$ & $58.2$ \\
        SwinV2-G~\cite{liu2021swinv2} & $3.0$B & SwinV2-G & IN-22K-ext-70M~\cite{liu2021swinv2} & - &   & $-$ & $-$ & $59.3$ & $59.9$\\
        \hline
        MASK DINO(Ours) & $\textbf{218}$\textbf{M} & SwinL & IN-22K-14M & O365 &   & $\textbf{59.1}$ & $\textbf{59.7}$ & $\textbf{-}$ & $\textbf{-}$ \\
        \midrule
    \end{tabular}
    \end{adjustbox}
    % }
    % \vspace{0.05cm}
    \caption{Comparison of the best detection models on MS-COCO. Similar to DETR~\cite{carion2020end}, we use the term ``end-to-end'' to indicate if a model is free from hand-crafted components like RPN and NMS. The term ``use mask'' means whether a model is trained with instance segmentation annotations. We use the terms ``IN'' and ``O365'' to denote the ImageNet~\cite{deng2009imagenet} and Objects365~\cite{shao2019objects365} datasets, respectively. Note that ``O365'' is a subset of ``FourODs'' and ``FLD-9M''. * DyHead does not disclose the details of the datasets used for model pre-training.
    }
    \label{tab:sota}
    % \vspace{-.6cm}
\end{table}
